BingoGuard: LLM Content Moderation Tools with Risk Levels

Malicious content generated by large language models (LLMs) can pose varying degrees of harm. Although existing LLM-based moderators can detect harmful content, they struggle to assess risk levels and may miss lower-risk outputs. Accurate risk assessment allows platforms with different safety thresholds to tailor content filtering and rejection. In this paper, we introduce per-topic severity rubrics for 11 harmful topics and build BingoGuard, an LLM-based moderation system designed to predict both binary safety labels and severity levels. To address the lack of annotations on levels of severity, we propose a scalable generate-then-filter framework that first generates responses across different severity levels and then filters out low-quality responses. Using this framework, we create BingoGuardTrain, a training dataset with 54,897 examples covering a variety of topics, response severity, styles, and BingoGuardTest, a test set with 988 examples explicitly labeled based on our severity rubrics that enables fine-grained analysis on model behaviors on different severity levels. Our BingoGuard-8B, trained on BingoGuardTrain, achieves the state-of-the-art performance on several moderation benchmarks, including WildGuardTest and HarmBench, as well as BingoGuardTest, outperforming best public models, WildGuard, by 4.3\%. Our analysis demonstrates that incorporating severity levels into training significantly enhances detection performance and enables the model to effectively gauge the severity of harmful responses.

==> tables/algorithm.tex <==
%<-- Wrapfigure covers 6 lines
\begin{wrapfigure}[22]{R}{0.6\textwidth}
\begin{minipage}{0.6\textwidth}
  \begin{algorithm}[H]
\caption{Iterative filter and refine algorithm}\label{alg:refine}
\begin{algorithmic}

\Require
$M$: moderator from last iteration;  
$M_1$, $M_2$: moderator committee; 
$\{q_i, r_i^{init}, r_i^2, r_i^3, r_i^4\}_{i=1}^N$: queries, initial responses, and candidate responses from other levels
\Ensure $\{q_i, r_i^{new}\}_{i=1}^N$: Refined dataset
\For{$i\gets 1, N$}
\State $r_i^{new} \gets r_i^{init}$
 \For{$j\gets 4, 2$}
     \If{$M\left(q_i, r_i^j\right) = 0$ and $\sum_{k=1,2} M_k\left(q_i, r_i^j\right) \geq 1$}
        \State $r_i^{new} \gets r_i^j$ \Comment{replace when at least one model from the committee label `unsafe'}
        \State \textbf{break}
    \EndIf
 \EndFor

\EndFor
\end{algorithmic}
\end{algorithm}  
\end{minipage}


\end{wrapfigure}

==> tables/calibration.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{lightgray}{gray}{0.9}
\begin{table*}[h]
\renewcommand{\arraystretch}{1.05}
\scalebox{1.0}{
\begin{tabular}[h]{p{2.28cm} | m{1.8cm}m{1.8cm}m{1.8cm}m{1.8cm}}
\toprule 
\bf & level1 & level2 & level3 & level4 \cr
\midrule
LlamaGuard3 & 0.91& 0.94& 0.94& 0.90\cr
MD-judge & 0.69 & 0.74& 0.86& 0.83\cr
BingoGuard & 0.91 & 0.92 & 0.94 & 0.99  \cr
\bottomrule
\end{tabular}}
\caption{Results on BingoGuard test set.}
\label{tab:ablation}
\end{table*}



==> tables/severityprinciple.tex <==
1. Intention: educational vs. mali intentional. Whether the response is provide educational information or provide direct malicious information. 2. Content: (meta) discussion-level vs. instruction-level vs. endorsement-level. Whether the response generally comments, instructs, or incites harmful behaviors. 3. Impact: individual vs. collective/social/cultural. Whether the response targets individuals or groups of people. 4. Context: context agnostic vs. context gnostic. Whether the response is harmful regardless of the context, or mostly benign but can be harmful based on the context. 5. Subjectivity: mention/statistics/documents/objectivity vs. opinions/subjectivity. Whether the response is describing something in an objective manner or gives subjective opinions. 6. Attitude: Negative/caveat/warning vs. neutral vs. positive/support. Does the response warns about, be neutral, or support harmful consequences 7. Graphic: non-graphical vs. graphical. Whether the description is graphic.

\begin{table*}[h]
\renewcommand{\arraystretch}{1.05}
\centering
\scalebox{1.0}{
\begin{tabular}[h]{p{2.28cm} | m{1.0cm}m{1.0cm} m{1.0cm}m{1.0cm}m{0.8cm}}
\toprule 
\bf & level1 & level2 & level3 & level4 & Avg. \cr
\midrule
LlamaGuard2 & 8.5& 39.7& 73.4& 65.6& 52.3 \cr
LlamaGuard3 & 10.2 & 46.4 & 77.3 & 75.3 & 58.6 \cr
MD-Judge & 17.2 & 62.3 & 90.3 & 90.4 & 72.3 \cr
WildGuard & 6.5 & 50.0 & 86.0 & 83.4 & 65.2 \cr
ShieldGemma \cr
GPT-4o \cr
\midrule
BingoGuard & 15.6 & 75.2 & 95.2 & 96.7 & 78.9 \cr
\bottomrule
\end{tabular}}
\caption{Results on BingoGuard test set.}
\label{tab:bingotest}
\end{table*}
